Diffusion for the periodic wind-tree model

The periodic wind-tree model is an infinite billiard in the plane with identical rectangular scatterers disposed at each integer point. We prove that independently of the size of the scatterers, generically with respect to the angle, the polynomial diffusion rate in this billiard is 2/3.

==> generic-surfaces-to-generic-parameters.tex <==
\section{From deviations for generic surfaces to deviations for $\Xsurf(a,b)$} \label{section:generic_surfaces_to_generic_windtree_parameters}
In this section we prove that Lemma~\ref{lem:deviations_for_almost_all_surfaces} implies Theorem~\ref{thm:divergence_rate_surface}. We emphasise that Lemma~\ref{lem:deviations_for_almost_all_surfaces} is a statement on deviations which is valid for a generic surface in $\Xablocus$ but not necessarily for the surfaces $r_\theta \Xsurf(a,b)$ which comes from the billiard unfolding (see section~\ref{section:from_infinite_billiard_to_finite_surface}). Using properties of the Teichm\"uller flow and the KZ cocycle we prove that the theorem actually holds for $r_\theta \Xsurf(a,b)$.

For the whole section, we fix a neighbourhood $U$ of the surfaces $\{r_\theta \Xsurf(a,b)\}_{\theta,a,b}$ in $\Xablocus$ on which the vector $f \in H^1(\Xsurf(a,b);\Z^2)$ may be globally defined. For a translation surface $Y \in U$ and $p \in Y$ we consider the function
\[
F(Y,p) = \limsup_{T \to \infty} \frac{\log | \langle f,\gamma_T(p),v \rangle |}{\log(T)}.
\]
We summarise what is already proven: the quantity $F(Y,p)$ is equal to $2/3$ for almost every $Y \in U$ and every $p \in Y$ with infinite orbit under the linear flow. The strategy to prove that $F(Y,p) = 2/3$ for the surfaces $r_\theta \Xsurf(a,b)$ is to prove that $F$ is constant along the leaf of a foliation $\WWW^s$. In a second time, we check that the set of surfaces $\{r_\theta \Xsurf(a,b)\}$ is a smooth transversal to $\WWW^s$ (lemmas~\ref{lem:Xabtheta-transversal-Tcurves} and~\ref{lem:Xabtheta-transversal-stratum}). The proof then follows from an application of Fubini theorem using that the foliation $\WWW^s$ and its transversal given by the surfaces $\{r_\theta \Xsurf(a,b)\}$ is smooth (Lemma~\ref{lem:regularity-foliation}) 

\begin{remark}
To simplify notations, in this section, the sentence {\it for every $p \in Y$} means {\it for every $p \in Y$ with infinite forward orbit}.
\end{remark}

Following~\cite{Fo2}, we define a foliation $\WWW^s$ on $\Xablocus$ invariant under the Teichm\"uller flow. For $X \in \Xablocus$, the leaf through $X$ is
\[
\WWW^s(X) = \{Y \in \Xablocus; \exists t_0 \in \R,\, \lim_{t \to \infty} d(g_t X, g_{t_0+t} Y) = 0\}.
\]
In other words, the set $\WWW^s(X)$ is the orbit of a strongly stable space under the geodesic flow. In a stratum the set $\WWW^s(X)$ is highly regular: it is defined by linear equations. More precisely, let $\omega$ be the Abelian differential that defines $X$. Then, $\WWW^s(X)$ is locally the set of Abelian differential $\omega'$ such that there exists $\alpha$ such that $\Re(\omega') = \alpha \Re(\omega)$. In other words, given a decomposition of a translation surface in zippered rectangle, the asymptotic of the forward Teichm\"uller geodesic is not modified by changing the heights of the rectangles.

\begin{lemma} \label{lem:invariance_of_F}
The function $F$ is constant along the leaves of the foliation $\WWW^s$.
\end{lemma}

\begin{proof}
From its definition, the function $F$ is invariant along a Teichm\"uller geodesic. Moreover, it follows from our proof that it only depends on the asymptotic of its Teichm\"uller geodesic (through the KZ cocycle).
\end{proof}

From section~\ref{sec:computation_of_Lyapunov_exponents}, we know that the list of $\SL(2,\R)$-ergodic measures on $\Xablocus$ consists in a family of $\SL(2,\R)$-ergodic measures supported on Teichm\"uller curves and the Lebesgue measure on $\Xablocus$. We first consider the case of the measure $\mu$ supported on a Teichm\"uller curve $\CCC$. In that case, the leaf $\WWW^s(X) \cap \CCC$ at a point $X \in \CCC$ is the orbit of the upper triangular matrices $P = \{g_t h_s X\}_{s \in \R, t \in \R}$. In other words, each leaf is modeled on $\R^2$.
\begin{lemma} \label{lem:Xabtheta-transversal-Tcurves}
Let $\CCC = \SL(2,\R) \cdot \Xsurf(a,b)$ be a Teichm\"uller curve in $\Xablocus$. The map $\theta \mapsto r_{\theta} \Xsurf(a,b)$ is locally a transversal to the foliation $\WWW^s \cap \CCC$ of $\CCC$.
\end{lemma}

\begin{proof}
From Iwasaw decomposition, there is a diffeomorphism $P \times K \rightarrow \SL(2,\R)$ where $P$ is the set of upper triangular matrix and $K = \{r_\theta\}_{\theta \in S^1}$. On the other hand, the Teichm\"uller curve $\CCC$ is isomorphic to the quotient $\SL(2,\R) / \Gamma$ where $\Gamma$ is the stabilizer of $\Xsurf(a,b)$. The local inverses of the map $\SL(2,\R) \rightarrow \CCC$ give local charts for $\CCC$. In particular, the $P$-orbit are transverse to the $K$-orbit and the lemma follows.
\end{proof}

We then consider the case of the Lesbegue measure on $\Xablocus$.
\begin{lemma} \label{lem:Xabtheta-transversal-stratum}
The map
\[
\begin{array}{ccc}
(0,1) \times (0,1) \times S^1  & \rightarrow & \Xablocus \\
(a,b,\theta,t) & \mapsto & r_\theta \Xsurf(a,b)
\end{array}
\]
is locally a transversal to $\WWW^s$ on $\Xablocus$.
\end{lemma}

\begin{proof}
We recall that the stratum $\HHH(2)$ has real dimension $8$ while $\HHH^{(1)}(2)$ denotes the set of translation surfaces in $\HHH(2)$ of area $1$ and hence has real dimension $7$. The set $\Xablocus$ is a finite cover of $\HHH^{(1)}(2)$ and the foliations $\WWW^s$ is well defined on the latter. The surfaces $r_\theta \Xsurf(a,b)$ maps to the surfaces $r_\theta \Lsurf(a,b)$ (see Section~\ref{section:background} and Figure~\ref{fig:Lab}). It is hence sufficient to prove the transversality of the family $r_\theta \Lsurf(a,b)$ in $\HHH^{(1)}(2)$.

In $\HHH^{(1)}(2)$, the leaves of $\WWW^s$ are modeled on $\R^4$ (which corresponds to the half of the dimension of $\HHH(2)$). Let $\omega_{a,b,\theta}$ be the area $1$ Abelian differential of the translation surface $r_\theta \Lsurf(a,b)$. A basis of $H_1(\Xsurf(a,b),\Z)$ is given by the sides $h_1$, $h_2$, $v_1$ and $v_2$ of $\Lsurf(a,b)$ seen on Figure~\ref{fig:Lab}. The integration of $\Re(\omega_{a,b,\theta})$ on that basis gives
\[ \Re(\omega_{a,b,\theta}) (h_1) = \frac{(1-a) \cos(\theta)}{\sqrt{1-ab}} \quad \Re(\omega_{a,b,\theta}) (h_2) = \frac{a \cos(\theta)}{\sqrt{1-ab}}\]
and
\[ \Re(\omega_{a,b,\theta}) (v_1) = \frac{(1-b) \sin(\theta)}{\sqrt{1-ab}} \quad \Re(\omega_{a,b,\theta}) (v_2) = \frac{b \sin(\theta)}{\sqrt{1-ab}}\]
We know that the integration of the Abelian differential on the homology $P: \HHH(2) \rightarrow H^1(S,\C)$ gives local charts to the stratum $\HHH^{(1)}(2)$. From its definition, the leaves of $\WWW^s$ in these chart are the fibers of $\Re \circ P$. From the above formulas and inverse function theorem, we get that the map $(a,b,\theta) \mapsto \Re(\omega_{a,b,\theta})$ is locally a diffeomorphism on its image and is hence a transversal to the foliation $\WWW^s$. 
\end{proof}

The foliation $\WWW^s$ provides a local product structure: the leaves are modeled on an euclidean space isomorphic to $\R^2$ in the case of a Teichm\"uller curve and $\R^4$ in the case of $\Xablocus$. The transversal is modeled on $\R$ in the case of Teichm\"uller curve (corresponding to the action of $r_\theta$) and $\R^3$ in the case of $\Xablocus$ (corresponding to the three parameters $(a,b,\theta)$). In order to apply Fubini theorem, we need some regularity which is the object of the following lemma.
\begin{lemma} \label{lem:regularity-foliation}
Let $\CCC = \SL(2,\R) \Xsurf(a,b)$ be a Teichm\"uller curve. Then the Haar measure on $\CCC$ is locally the product measure of the Lebesgue measure on the leaf and the Lebesgue measure on the transversal.

The Lebesgue measure on $\Xablocus$ is locally the product measure of the Lesbegue measure on the leaves of $\WWW^s$ and a measure absolutely continuous with respect to Lebesgue on the transversal.
\end{lemma}

\begin{proof}
The case of the Haar measure is quite clear as the map $P \times K \rightarrow \SL(2,\R)$ is smooth and the Haar measures in $\SL(2,\R)$ is the product of the Haar measure on $P \times K$.

The Lebesgue measure on $\HHH(2)$ is built by locally pulling back the Lebesgue measure from the period coordinates obtained by the integration of Abelian differentials. In particular, as the foliation $\WWW^s$ is linear in the coordinates and the transversal is smooth the Lebesgue measure decomposes as a product of the Lebesgue measure and a measure absolutely continuous to Lebesgue. Notice that the latter one can be made explicit from the computations of $\Re(\omega_{a,b,\theta})$ in the proof of Lemma~\ref{lem:Xabtheta-transversal-stratum}.
\end{proof}

We now recall the standard argument using Fubini theorem that Lemma~\ref{lem:deviations_for_almost_all_surfaces} implies Theorem~\ref{thm:divergence_rate_surface}. We only prove it for the whole stratum as the arguments are identical for Veech curves. By taking $U$ smaller we may consider that it is a flow box $U \simeq U_1 \times U_2$ in $\Xablocus$ where $U_1$ is an open set in $\R^4$ and $U_2$ is an open set of parameters $(a,b,\theta)$. Then, we know that for almost all surfaces in $U$ the function $F$ is constant equals to $2/3$. Now, by Lemma~\ref{lem:regularity-foliation} and Fubini theorem, a set of full measure in $U$ has projections of full measure in both $U_1$ and $U_2$. As from Lemma~\ref{lem:invariance_of_F} the function $F$ is invariant along the leaf, $F$ is $2/3$ for almost every $(a,b,\theta) \in U_2$.

